Diagnosing Vision-and-Language Navigation: What Really Matters

Vision-and-language navigation (VLN) is a multimodal task where an agent follows natural language instructions and navigates in visual environments. Multiple setups have been proposed, and researchers apply new model architectures or training techniques to boost navigation performance. However, there still exist non-negligible gaps between machines' performance and human benchmarks. Moreover, the agents' inner mechanisms for navigation decisions remain unclear. To the best of our knowledge, how the agents perceive the multimodal input is under-studied and needs investigation. In this work, we conduct a series of diagnostic experiments to unveil agents' focus during navigation. Results show that indoor navigation agents refer to both object and direction tokens when making decisions. In contrast, outdoor navigation agents heavily rely on direction tokens and poorly understand the object tokens. Transformer-based agents acquire a better cross-modal understanding of objects and display strong numerical reasoning ability than non-Transformer-based agents. When it comes to vision-and-language alignments, many models claim that they can align object tokens with specific visual targets. We find unbalanced attention on the vision and text input and doubt the reliability of such cross-modal alignments.

==> response.tex <==
\section*{Response to Sep.15th ACL RR Reviews}

We thank the reviewers for their insightful feedback! We are encouraged that reviewers find our experiments clearly designed and executed(\rac, \rtwo, \rthree, \rfour), displaying surprising findings(\rone), 
providing comparison on several models(\rac, \rtwo, \rthree), andmotivating VLN researchers to further explore model behavior, which eventually may lead to insights that improve the navigation performance of these systems(\rone). 

We incorporated all feedback and revised our submission. We address reviewers' comments below, and enclose a version of our draft in which the major modifications are highlighted.


%----------------------
\rquestion{\rac, @\rfour}{Train-Test Distribution Shift}
We agree that ablating the validation data will result in the distribution shift from the training data. However, such distribution shift indeed provides an opportunity to study the models' robustness and the ability to generalize to unseen environment, which is a major problem in VLN research~\cite{DBLP:conf/emnlp/LiLXBCGSC19,DBLP:conf/naacl/TanYB19}. 
Moreover, recent studies on model performance analysis have also apply similar ablations on input data during validation. We noted this in Section~\ref{q:distribution_shift} (line 104-202).


%----------------------
\rquestion{\rac, @\rone, @\rfour}{Discussion of Performance Trends}
Thanks for the suggestion. We remove the claim on ``VLN reaching performance ceiling'', and change it into a more objective report on the performance gaps between machines and humans on VLN datasets in Figure~\ref{tab:human_sota_comparison}.

%----------------------
\rquestion{\rac, @\rfour}{Discussion of Heuristics}
Thanks for the suggestion. We discuss the accuracy of the heuristic model used in our study in Section~\ref{sec:heuristics}.
There exists a few cases where the object token labels generated by the heuristic part-of-speech tagging model disagree with human annotations. However, the misalignment occurs infrequently. Thus, we continue to use heuristic model to detect object tokens in our study.

%----------------------
\rquestion{\rac, @\rfour}{Bias on R2R}
Thanks for pointing out! We include the experiments on the RxR dataset~\cite{rxr} in the revision, and compare navigation performance on CLIP-ViL~\citep{Shen2021HowMC} and VLN-HAMT~\citep{chen2021hamt}. Please refer to Section~\ref{sec:instr}, ~\ref{sec:visual_env} and ~\ref{sec:vision_language_alignment} for in-depth discussion.


%----------------------
\rquestion{\rac, @\rone, @\rtwo, @\rthree, @\rfour}{Presentation}
Thanks for pointing this out! We remove all the tiny figures, and display the results in Tables for clearer presentation.


%----------------------
\rquestion{\rone}{Discussion on Mentioned Models}
Thanks for pointing this out! 
We include more discussions on the mentioned models in the revision. 
In short, we find out that Transformer-based models have relatively better understanding on both text and visual input, and is more robust to ablations on input data. In addition, we notice that the backbone to extract visual features from the environment also matters. 

For discussions on model structure, please refer to Table~\ref{tab:tasks_datasets} and Section~\ref{sec:align_instr}.
For discussion on visual features, please refer to Section~\ref{sec:instr_object} (line 359-365) and Section~\ref{sec:visual_env} (line 492-510).

%----------------------
\rquestion{\rone}{Performance difference between Indoor \& outdoor agents} 
The differences are more caused by dataset properties and visual features. 
In short, the reasons are two-fold. First, the search space for ourdoor VLN on Touchdown is more extensive than indoor VLN, which we discuss in Section~\ref{q:indoor_outdoor_difference_1}. Second, current indoor agents use features extracted by ResNet-152 or CLIP-ViT, while outdoor agents use ResNet-18 to extract visual features, which is not powerful enough to encode all visual information in the complicated urban environment. We discuss this in Table~\ref{tab:tasks_datasets} and Section~\ref{sec:instr_object} (line 359-365).

%----------------------
\rquestion{\rone}{Fine-grained Analysis of Constructions for Directions}
Thanks for the suggestion! We add a discussion on agents' ability to count in Section~\ref{sec:instr_count}. We notice that indoor agents have the ability to count to some extent on the RxR dataset, while outdoor agents don't.

%----------------------
\rquestion{\rone}{Explain R2R and Touchdown}
Thanks for the suggestion! We add reference to R2R, RxR and Touchdown in Section ~\ref{q:explain_dataset} (line 107-109).


%----------------------
\rquestion{\rone}{"without loss of generality"}
Sorry for causing confusion. We removed this line in revison.


%----------------------
\rquestion{\rone}{Explain Success Rate and Task Completion metrics}
Thanks for the suggestion! We explain the definition of Success Rate and Task Completion in Section~\ref{sec:metric} (line 266-277).

%----------------------
\rquestion{\rone}{Provide the number of object and direction tokens as a percentage}
Thanks for the suggestion! We addressed this in Table~\ref{tab:dataset_comparison}.

%----------------------
\rquestion{\rone}{Explain object-related and direction-related tokens}
We explained this in Section~\ref{sec:instr_object} (line 319-321) and Section~\ref{sec:instr_direction} (line 367-369). Table~\ref{tab:instr_examples} provides examples of object and direction tokens.


%----------------------
\rquestion{\rone}{What it means by "Noticeably, when we mask out the object tokens, the tokens visible to the agent also decrease, which is a coherent factor with \#object tokens and might interfere with our analysis."}
Take Table~\ref{tab:masking_examples} as an example. The vanilla instruction contains 31 tokens. After masking out all the six object tokens, there are only 25 visible tokens in the instruction. The loss of visible tokens may also decrease the results. We justify this by adding a controlled trial, where six random tokens are masked out.

%----------------------
\rquestion{\rone}{Bring related work section forward}
We happily followed this advice and bring the related work to Section~\ref{sec:related_work}

%----------------------
\rquestion{\rtwo}{Tables in Appendix}
Sorry for causing confusion. We removed the big tables in appendix.

%----------------------
\rquestion{\rtwo}{Explain the various effects in more detail}

Thanks for the suggestion! We followed your advice in the revision.  Please refer to Section~\ref{sec:instr}, ~\ref{sec:visual_env} and ~\ref{sec:vision_language_alignment} for in-depth discussion.



% %----------------------
% \rquestion{\rtwo}{Test complex semantic and compositional phenomena}



%----------------------
\rquestion{\rtwo}{Tokens other than object/direction}

Thanks for the suggestion! We add a discussion on agents' ability to count in Section~\ref{sec:instr_count}. We notice that indoor agents have the ability to count to some extent on the RxR dataset, while outdoor agents don't.


%----------------------
\rquestion{\rtwo}{Focus on "highlights" }

Thanks for the suggestion! We followed your advice in the revision and removed not-so-exciting findings from the main paper.  Please refer to Section~\ref{sec:instr}, ~\ref{sec:visual_env} and ~\ref{sec:vision_language_alignment} for in-depth discussion.

% %----------------------
% \rquestion{\rthree}{The placement of the background vs. foreground objects}
% We explain the definition of 



%----------------------
\rquestion{\rthree}{Making summary comparisons easier}

Thanks for the suggestion! We followed your advice in the revision, and display related results in the same table for easier comparisons.  Please refer to Section~\ref{sec:instr}, ~\ref{sec:visual_env} and ~\ref{sec:vision_language_alignment} for in-depth discussion.


%----------------------
\rquestion{\rthree}{Adding additional control experiments or justification}

Thanks for the suggestions! We add additional justifications in the revision. Please refer to Section~\ref{sec:visual_env} (line 492-510).

% %----------------------
% \rquestion{\rfour}{Paper writing}

% Thanks for the suggestion! We followed your advice in the revision.

%----------------------
\rquestion{\rfour}{Technical details of the procedure in Section 4.1}

Thanks for asking! We explain the technical details of visual environment ablations in Section~\ref{sec:visual_env} (line 445-472).
